Counting Immutable Beans: Reference Counting Optimized for Purely Functional Programming

Most functional languages rely on some garbage collection for automatic memory management. They usually eschew reference counting in favor of a tracing garbage collector, which has less bookkeeping overhead at runtime. On the other hand, having an exact reference count of each value can enable optimizations, such as destructive updates. We explore these optimization opportunities in the context of an eager, purely functional programming language. We propose a new mechanism for efficiently reclaiming memory used by nonshared values, reducing stress on the global memory allocator. We describe an approach for minimizing the number of reference counts updates using borrowed references and a heuristic for automatically inferring borrow annotations. We implemented all these techniques in a new compiler for an eager and purely functional programming language with support for multi-threading. Our preliminary experimental results demonstrate our approach is competitive and often outperforms state-of-the-art compilers.

==> alloc.tex <==
Memory allocation is very efficient in garbage collectors used in
state-of-the-art compilers such as ocamlopt and ghc. The OCaml garbage
collector is a modern hybrid generational and incremental collector
that is known to often outperform manual memory
allocation. Generational garbage collectors also improve cache
locality~\cite{ZornGC} which is an important feature for modern
hardware architectures where poor locality often reduces program
performance~\cite{cachelocality}.

We initially used the standard \emph{malloc} and \emph{free} from the C standard library to implement
our runtime, and have observed poor performance in many benchmarks.
Profiling data made it clear that \emph{malloc} and \emph{free} were the bottlenecks.
We addressed this issue by switching to \emph{jemalloc}~\cite{jemalloc}, a \emph{malloc}
and \emph{free} replacement, and have observed a significant performance
improvement in many benchmarks by up to 3x. We obtained another $30\%$
performance improvement by implementing our own custom memory allocator
optimized for small values. Our allocator uses a new memory allocation
technique developed by \citet{freelistsharding} for the Koka programming
language~\cite{Koka} runtime.

We have also implemented lazy reference counting as a configuration option
in our runtime for users that might be concerned with long pauses when
deallocating values. The idea is quite simple: The instruction
$\kw{dec}\ x$ just puts $x$ in a deletion queue if its reference count
becomes $0$.  Before we allocate memory, we check the deletion queue,
and remove one value if it is not empty, and invoke $\kw{dec}$ on
nested values. \citet{BoehmCostRC} shows that lazy reference
counting may result in an unacceptable worst-case space overhead. We
did not manage to observe the worst-case behavior in any of our
benchmarks, but further investigation is needed. We suspect that
providing a primitive for (partially) flushing the lazy reference
counting queue should be sufficient to address any program that may
experience a significant space overhead.

